Providing Real-time Assistance for Repairing Runtime Exceptions using Stack Overflow Posts

Runtime Exceptions (REs) are an important class of bugs that occur frequently during code development. Traditional Automatic Program Repair (APR) tools are of limited use in this "in-development" use case, since they require a test-suite to be available as a patching oracle. Thus, developers typically tend to manually resolve their in-development REs, often by referring to technical forums, such as Stack Overflow (SO). To automate this manual process we extend our previous work, MAESTRO, to provide real-time assistance to developers for repairing Java REs by recommending a relevant patch-suggesting SO post and synthesizing a repair patch from this post to fix the RE in the developer's code. MAESTRO exploits a library of Runtime Exception Patterns (REPs) semi-automatically mined from SO posts, through a relatively inexpensive, one-time, incremental process. An REP is an abstracted sequence of statements that triggers a given RE. REPs are used to index SO posts, retrieve a post most relevant to the RE instance exhibited by a developer's code and then mediate the process of extracting a concrete repair from the SO post, abstracting out post-specific details, and concretizing the repair to the developer's buggy code. We evaluate MAESTRO on a published RE benchmark comprised of 78 instances. MAESTRO is able to generate a correct repair patch at the top position in 27% of the cases, within the top-3 in 40% of the cases and overall return a useful artifact in 81% of the cases. Further, the use of REPs proves instrumental to all aspects of MAESTRO's performance, from ranking and searching of SO posts to synthesizing patches from a given post. In particular, 45% of correct patches generated by MAESTRO could not be produced by a baseline technique not using REPs, even when provided with MAESTRO's SO-post ranking. MAESTRO is also fast, needing around 1 second, on average, to generate its output.

==> acknowledgments.tex <==
\section*{acknowledgments}
We would like to express our gratitude for the significant time and effort invested by our two participants, who evaluated several hundred \ac{so} posts and provided the relevancy ratings for RQ1--3. We also thank the participants of our user experience case study for their valuable feedback. Finally, thanks to the anonymous reviewers for their constructive input, which helped improve the quality of this manuscript.
